PIGLeT: Language Grounding Through Neuro-Symbolic Interaction in a 3D World

We propose PIGLeT: a model that learns physical commonsense knowledge through interaction, and then uses this knowledge to ground language. We factorize PIGLeT into a physical dynamics model, and a separate language model. Our dynamics model learns not just what objects are but also what they do: glass cups break when thrown, plastic ones don't. We then use it as the interface to our language model, giving us a unified model of linguistic form and grounded meaning. PIGLeT can read a sentence, simulate neurally what might happen next, and then communicate that result through a literal symbolic representation, or natural language. Experimental results show that our model effectively learns world dynamics, along with how to communicate them. It is able to correctly forecast "what happens next" given an English sentence over 80% of the time, outperforming a 100x larger, text-to-text approach by over 10%. Likewise, its natural language summaries of physical interactions are also judged by humans as more accurate than LM alternatives. We present comprehensive analysis showing room for future work.

==> figures/counts_fig.tex <==
\begin{figure*}[t!]
\centering\small
\begin{minipage}{.47\textwidth}
  \centering\small
  \includegraphics[width=\linewidth]{figures/conceptcounts.pdf}\vspace{5mm}
  \captionof{figure}{Counts of zero-shot words that appear in BERT's training data (Wikipedia and Toronto Books). For example, in the 4 billion words BERT is trained on, it sees the word `Bed' almost 500k times. This might allow it to perform superficially well at answering questions about beds -- while not necessarily possessing deep physical knowledge about them.}
  \label{fig:conceptcounts}
\end{minipage}%
\hspace{.059\textwidth}\begin{minipage}{.47\textwidth}%\vspace*{-3mm}
  \centering\small
  \includegraphics[width=\linewidth]{figures/nwords.pdf}%\vspace*{-2mm}
  \captionof{figure}{Size of the pretraining datasets used by today's large language models. The datasets used are getting exponentially larger with time, with GPT3's training dataset containing over half a trillion words. In contrast, a child of high socioeconomic status is exposed to 21k words per day, or roughly 40M words by age five \citep{fernald2013wordcounts}.
  }
  \label{fig:pretraindatasetsizes}
\end{minipage}
\end{figure*}


==> figures/t_questions.tex <==
\begin{table}[t]
    \footnotesize\centering{\frenchspacing\renewcommand{\arraystretch}{1.4}
    \begin{tabular}{@{}p{7.4cm} @{\hspace{0.2cm}} p{3cm} @{\hspace{0.1cm}} p{3cm} @{}}
        \toprule
        Statement template & Example true objects & Example false objects \\[-0.05cm]
        \midrule
        \cmidrule{1-3}
        I can cook \blankthorobject{[object]}. & \thorobject{Egg}, \thorobject{Potato}, \ldots &  \thorobject{Bottle}, \thorobject{Toilet}, \ldots \\
        I can use a kitchen knife to slice \blankthorobject{[object]}. &  &  \\
        I can put objects (the size of an apple or larger) in/on \blankthorobject{[object]}. &  &  \\
        \blankthorobject{[object]}s are often partially made of \thormaterial{[material]}. &  &  \\
        I can turn \blankthorobject{[object]} on or off. &  &  \\
        I can fill \blankthorobject{[object]} with liquid using a kitchen faucet. &  &  \\
        If I drop \blankthorobject{[object]}, it would likely break. &  &  \\
        If I throw \blankthorobject{[object0]} at \blankthorobject{[object1]} hard enough,   \blankthorobject{[object1]} would likely break. &  &  \\
        I can put \blankthorobject{[object0]} in/on \blankthorobject{[object1]}. &  &  \\
        I might be able to heat up \blankthorobject{[object0]} by putting it in/on \blankthorobject{[object1]}. &  &  \\
        I can clean a dirty \blankthorobject{[object0]} in/on \blankthorobject{[object1]}. &  &  \\
        I can pick up \blankthorobject{[object]} by myself. &  &  \\
        I can fill \blankthorobject{[object0]} with liquid by putting it under \blankthorobject{[object1]}. &  &  \\
        I'd expect \blankthorobject{[object0]} to be heavier than \blankthorobject{[object1]}. &  &  \\
         \bottomrule
    \end{tabular}}
    \caption{Source templates for our questionnaire, \mcname. A model must answer `true' when the templates are instantiated with true objects (that were collected through THOR and verified by crowd workers), and vice versa for false objects. A model must also answer correctly for negations of the templates (e.g. I can't cook \protect\blankthorobject{[object]}), for which the sets of true and false objects are switched. Our evaluation paradigm and dataset challenge language-understanding systems to answer these questions correctly, even when they are not allowed to pretrain on physical-only words like \protect\thorobject{Egg}.}
    \label{tab:tfquestions}
\end{table}


==> figures/t_thor_full.tex <==
\begin{table*}[t]
    \footnotesize\centering{\frenchspacing\renewcommand{\arraystretch}{1.1}
    \begin{tabular}{@{}p{1.6cm} p{7.3cm} @{\hspace{0.4cm}} p{4.2cm}@{}}
        \toprule
        Generator & Description & Interesting outcomes \\[-0.05cm]
        \cmidrule{1-3}
        \thorfunction{put X in Y} & Samples an object \blankthorobject{X} from the scene, and a receptacle \blankthorobject{Y}. With probability $p{=}0.5$ toggles or slices \blankthorobject{X}, then tries to put it in \blankthorobject{Y}. & The object can change temperature, e.g., if we put it in a \thorobject{Fridge}. The action can fail or succeed.\\
        \thorfunction{throw X at Y} & Samples two objects \blankthorobject{X} and \blankthorobject{Y} from the scene. Picks up \blankthorobject{X}, moves to face \blankthorobject{Y}, and throws it forward with variable intensity. & An object can break. \\
        \thorfunction{toggle X} & Samples an object \blankthorobject{X}, and turns it on or off in the case of a \thorobject{LightSwitch} or an appliance. & An object can change state. \\
        \thorfunction{slice X} & Samples an object \blankthorobject{X} and a cutting surface \blankthorobject{Y} (like a \thorobject{CounterTop}). Picks up \blankthorobject{X}, places it on \blankthorobject{Y}, and cuts it. & The object can become sliced.\\
        % \thorfunction{dirty X} & Samples an object \blankthorobject{X}, and makes it dirty. & The object changes state. \\
        \thorfunction{clean X} & Samples a dirty object \blankthorobject{X}. Finds a \thorobject{Sink} nearby a \thorobject{Faucet}, and places \blankthorobject{X} inside. With probability (with probability $p{=}0.9$, turns on and off the \thorobject{Faucet}, cleaning the object. Last, tries to put \blankthorobject{X} away in a receptacle \blankthorobject{Y}. & The object becomes clean, unless we forget to turn on the \thorobject{Faucet}. \\
        \thorfunction{toast bread} & Finds some \thorobject{Bread}, slicing it if necessary. Places it in a \thorobject{Toaster}. With probability $p{=}0.9$, turns on/off the toaster, toasting the \thorobject{Bread}. & The \thorobject{Bread} changes state, unless we forgot to turn on or off the \thorobject{Toaster}. \\
        \thorfunction{brew coffee} & Picks up a \thorobject{Mug} and places it under a \thorobject{CoffeeMachine}. With probability $p{=}0.9$, turns on/off the coffee machine, filling the \thorobject{Mug}. & The \thorobject{Mug} changes state, unless we forgot to turn on the machine. \\
        \thorfunction{fry X} & Picks up a cookable object \blankthorobject{X} and slices it if necessary. Places it on a \thorobject{Pot} or \thorobject{Pan} and brings it to a \thorobject{StoveBurner}. Turns on the burner, cooking the object. & The object changes state, possibly several times -- for example, an \thorobject{Egg} is cracked, and then cooked. \\ 
        \thorfunction{microwave X} & Picks up an object \blankthorobject{X} and slices it if necessary. Places it in a \thorobject{Microwave} and closes it, then with probability $p{=}0.9$, turns it on or off. & Some objects get cooked, for others (such as a \thorobject{CD}), we learn that they do not belong there. \\
        \thorfunction{fill X} & Picks up an object \blankthorobject{X} places it under a \thorobject{Faucet}. With probability $p{=}0.9$, turns on/off the \thorobject{Faucet} Last, optionally pours out liquid in \blankthorobject{X}. & The object changes state (how much liquid is held).  \\
         \bottomrule
    \end{tabular}}
    \caption{Trajectory generation functions that we used to sample `interesting' physical interactions, such as the effects that actions will have on objects, and which actions will succeed or not.}
    \label{tab:thortrajectoryfns}
\end{table*}

